Prompt-driven Universal Model for View-Agnostic Echocardiography Analysis

Echocardiography segmentation for cardiac analysis is time-consuming and resource-intensive due to the variability in image quality and the necessity to process scans from various standard views. While current automated segmentation methods in echocardiography show promising performance, they are trained on specific scan views to analyze corresponding data. However, this solution has a limitation as the number of required models increases with the number of standard views. To address this, in this paper, we present a prompt-driven universal method for view-agnostic echocardiography analysis. Considering the domain shift between standard views, we first introduce a method called prompt matching, aimed at learning prompts specific to different views by matching prompts and querying input embeddings using a pre-trained vision model. Then, we utilized a pre-trained medical language model to align textual information with pixel data for accurate segmentation. Extensive experiments on three standard views showed that our approach significantly outperforms the state-of-the-art universal methods and achieves comparable or even better performances over the segmentation model trained and tested on same views.

==> tmp.tex <==

\begin{algorithm}
  \caption{Training procedure with prompt pool}
  \label{alg:training step}
  \Required{Initialize parameters of Segment Anything Model, $\mathcal{M}_{Q}$; Initialize prompt pool, $\mathcal{P}$ with learnable key and value, $(K, \mathbf{p})$}
  \KwIn{videos $x_1, ..., x_n $ and corresponding masks $y_1, ..., y_n$ from batch}
  \KwOut{trained models $f_\theta$}

  \For{$i=0,1,2,...,n-1$}
  {
    $f_q \leftarrow \mathcal{M}_{Q} \circ x_i$ \\
    
    \If{$x_i \in \{v_k \mid v_k \in \{A2C, A4C, PSAX\}\}$}
    {
      $sidx = \{0,1,2,3\} \times k$
    }
    
    $K \leftarrow K_{sidx}$ \\
    $L_{sim} \leftarrow \left\langle  \ \text{norm}(f_q), \text{norm}(K) \right\rangle \\
    $f_{\text{sample}} \leftarrow \text{GAP}(f_e(x), p)$ \\
    $L_{BCE} \leftarrow \text{\( \mathcal{L}_{seg} \)}(\ldots, \text{norm}(K))$ in Sec_{2.5}\\
    $L \leftarrow L_{sim} + L_{BCE}$ \\
    $\theta \leftarrow \arg\min_{\theta} L$ \\
  }
\end{algorithm}
